Indicators of Attack Failure: Debugging and Improving Optimization of Adversarial Examples

Evaluating robustness of machine-learning models to adversarial examples is a challenging problem. Many defenses have been shown to provide a false sense of robustness by causing gradient-based attacks to fail, and they have been broken under more rigorous evaluations. Although guidelines and best practices have been suggested to improve current adversarial robustness evaluations, the lack of automatic testing and debugging tools makes it difficult to apply these recommendations in a systematic manner. In this work, we overcome these limitations by: (i) categorizing attack failures based on how they affect the optimization of gradient-based attacks, while also unveiling two novel failures affecting many popular attack implementations and past evaluations; (ii) proposing six novel indicators of failure, to automatically detect the presence of such failures in the attack optimization process; and (iii) suggesting a systematic protocol to apply the corresponding fixes. Our extensive experimental analysis, involving more than 15 models in 3 distinct application domains, shows that our indicators of failure can be used to debug and improve current adversarial robustness evaluations, thereby providing a first concrete step towards automatizing and systematizing them. Our open-source code is available at: https://github.com/pralab/IndicatorsOfAttackFailure.

==> checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss the limitations in Sect.~\ref{sec:concl}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{In Sect.~\ref{sec:concl}, we specified that the aim of our work is not to break defenses in an harmful way. Our purpose is only to help researchers improving their security evaluation.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code will be submitted as supplementary material, and the instructions for reproducing the experiments are described in Sect.~\ref{sec:comparison-of-different-attacks}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We describe the experimental protocol in Sect.~\ref{sec:comparison-of-different-attacks}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{The resourced used for the experiments are listed in Sect.~\ref{sec:comparison-of-different-attacks}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited all the existing assets used for the experiments.}
  \item Did you mention the license of the assets?
    \answerYes{We cited the authors of the assets, and we provide the list of external assets along with the code.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide the code for computing the metrics as supplementary material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All the assets we used are publicly available.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> indicators_table.tex <==
\begin{table*}[]
\centering
\begin{tabular}{rcrrrrrrr}
\textbf{Model} &
  \textbf{Attack} &
  \textbf{\idc{1}} &
  \textbf{\idc{2}} &
  \textbf{\idc{3}} &
  \textbf{\idc{4}} &
  \textbf{\idc{5}} &
  \textbf{$\bar I$} &
  \multicolumn{1}{c}{\textbf{RA}} \\ \hline
                       & PGD         & 0.33 & 0.43 & 0.77 & -   & -& 0.306 & 58\% \\
\textit{k-WTA}~\cite{xiao2019resisting}         & APGD        & -   & 0.31 & 0.33 & -   & -& 0.128 & 36\% \\
                       & PGD$^\star$ & 0.07 & 0.48 & 0.55 & -   & -& 0.220  & 6\% \\ \hline
                       & PGD         & -   & 0.98 & -   & 0.97 & -& 0.39  & 94\% \\
\textit{Distillation}~\cite{papernot16-distill}  & APGD        & -   & 0.40  & 0.21 & -   & -& 0.122 & 0\% \\
                       & PGD$^\star$ & -   & 0.04 & -   & -   & -& 0.008 & 0\%    \\ \hline
                       & PGD         & -   & 0.76 & -   & -   & -& 0.152 & 38\%  \\
\textit{Ensemble Div.}~\cite{pmlr-v97-pang19a} & APGD        & -   & 0.37 & 0.14 & -   & - & 0.102 & 0\%     \\
                       & PGD$^\star$ & 0.08 & 0.17 & 0.15 & -   & -& 0.080  & 9\%  \\ \hline
 &
  PGD &
  -&
  0.49 &
  0.07 &
  -&
  0.37 &
  0.186&
  35\% \\ 
\textit{TWS}~\cite{Yu_2019_NeurIPSweakness}           & APGD        & -   & 0.41 & 0.09 & -   & -& 0.100   & 0\%     \\
                       & PGD$^\star$ & -   & 0.37 & 0.10  & -   & -& 0.094 & 0\%
\end{tabular}
\caption{Values of the Indicators of Attack Failures, computed for all the attacks against all the evaluated models. We denote the attacks that apply also the mitigations as PGD$^\star$.}
\label{table:all_indicators}
\end{table*}
